HybridSDF: Combining Deep Implicit Shapes and Geometric Primitives for 3D Shape Representation and Manipulation

Deep implicit surfaces excel at modeling generic shapes but do not always capture the regularities present in manufactured objects, which is something simple geometric primitives are particularly good at. In this paper, we propose a representation combining latent and explicit parameters that can be decoded into a set of deep implicit and geometric shapes that are consistent with each other. As a result, we can effectively model both complex and highly regular shapes that coexist in manufactured objects. This enables our approach to manipulate 3D shapes in an efficient and precise manner.

==> tex/defs.tex <==
% !TEX root = top.tex
% !TEX spellcheck = en-US

\newif\ifdraft
\draftfalse
%\drafttrue

\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{green0}{rgb}{0.1,0.7,0.1}
\newcommand{\sparag}[1]{\vspace{-3mm}\subparagraph{#1}}
\newcommand{\parag}[1]{\vspace{-1mm}\paragraph{#1}}

\ifdraft
 \newcommand{\PF}[1]{{\color{red}{\bf PF: #1}}}
 \newcommand{\pf}[1]{{\color{red} #1}}
 \newcommand{\SV}[1]{{\color{blue}{\bf SV: #1}}}
 \newcommand{\sv}[1]{{\color{blue} #1}}
 \newcommand{\NT}[1]{{\color{green0}{\bf NT: #1}}}
 \newcommand{\nt}[1]{{\color{green0} #1}}
\else
 \newcommand{\PF}[1]{{\color{red}{}}}
 \newcommand{\pf}[1]{ #1 }
 \newcommand{\SV}[1]{{\color{blue}{}}}
 \newcommand{\sv}[1]{ #1 }
 \newcommand{\NT}[1]{{\color{green0}{}}}
 \newcommand{\nt}[1]{ #1 }
\fi

% arXiv version (default is false)
\newif\ifarxiv
\arxivfalse
% If arXiv, can hyperlink reference to appendix, otherwise manually enter ref
\newcommand{\refappendix}[2]{\ifarxiv\ref{#1}\else#2\fi}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}

\newcommand{\bL}[0]{\mathcal{L}}
\newcommand{\bd}[0]{\mathbf{d}}
\newcommand{\by}[0]{\mathbf{y}}
\newcommand{\hby}[0]{\hat{\mathbf{y}}}

\newcommand{\real}{\mathbb{R}}

\newcommand{\PP}{\mathrm{PP}}
\newcommand{\AP}{\mathrm{AP}}
\newcommand{\TP}{\mathrm{TP}}
\newcommand{\IoU}{\mathrm{IoU}}

\newcommand{\ha}[0]{\hat{a}}
\newcommand{\hb}[0]{\hat{b}}

%\newcommand{\comment}[1]{}

%Algos
\newcommand{\CCQ}{{\it CCQ}}
\newcommand{\TLTS}{{\it TLTS}}
\newcommand{\APLS}{{\it APLS}}
\newcommand{\HM}{{\it H\&M}}


% new adds
\newcommand{\bp}[0]{\textbf{p}}
\newcommand{\mbp}[0]{\mathbf{p}}
\newcommand{\SDF}[0]{\mathbf{SDF}}
\newcommand{\LC}[0]{\mathbf{LC}}
\newcommand{\LV}[0]{\mathbf{LV}}

\newcommand{\lcp}{{$\mathbf{LC}_{\text{part}}$}}
\newcommand{\bR}[0]{\textbf{R}}
\newcommand{\bT}[0]{\textbf{T}}
\newcommand{\bS}[0]{\textbf{S}}

\newcommand{\DeepS}{{\it DeepSDF}}
\newcommand{\DeepSV}{{\it DeepSDF-V}}
\newcommand{\HS}{{\it HybridSDF}}
\newcommand{\HSV}{{\it HybridSDF-V}}
\newcommand{\HSs}{{\it HybridSDF$_{s}$}}
\newcommand{\HSd}{{\it HybridSDF$_{d}$}}
\newcommand{\HSVs}{{\it HybridSDF-V$_{s}$}}
\newcommand{\HSVd}{{\it HybridSDF-V$_{d}$}}
\newcommand{\HSb}{{\it HybridSDF$_{base}$}}
\newcommand{\DualS}{{\it DualSDF}}
\newcommand{\NP}{{\it NeuralParts}}
\newcommand{\HSQ}{{\it HierSQ}}
